A Sober Look at LLMs for Material Discovery: Are They Actually Good for Bayesian Optimization Over Molecules?

Automation is one of the cornerstones of contemporary material discovery. Bayesian optimization (BO) is an essential part of such workflows, enabling scientists to leverage prior domain knowledge into efficient exploration of a large molecular space. While such prior knowledge can take many forms, there has been significant fanfare around the ancillary scientific knowledge encapsulated in large language models (LLMs). However, existing work thus far has only explored LLMs for heuristic materials searches. Indeed, recent work obtains the uncertainty estimate -- an integral part of BO -- from point-estimated, non-Bayesian LLMs. In this work, we study the question of whether LLMs are actually useful to accelerate principled Bayesian optimization in the molecular space. We take a sober, dispassionate stance in answering this question. This is done by carefully (i) viewing LLMs as fixed feature extractors for standard but principled BO surrogate models and by (ii) leveraging parameter-efficient finetuning methods and Bayesian neural networks to obtain the posterior of the LLM surrogate. Our extensive experiments with real-world chemistry problems show that LLMs can be useful for BO over molecules, but only if they have been pretrained or finetuned with domain-specific data.

==> contents/99_apndx_notes.tex <==
%!TEX root=../main.tex

\section*{Finding 1: Results with fixed features}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.5\linewidth]{figs/diagram_fixed_feat}

	\caption{\textbf{Source of uncertainty:} The BNN regressor. Already more principled than the uncertainty of ICL.}
\end{figure}

Datasets:
\vspace{-1em}
\begin{itemize}
	\small
	\item \textbf{Redoxmer}: 1406 molecules, minimizing redox potential.
	\item \textbf{Solvation}: 1406 molecules, minimizing solvation energy.
\end{itemize}

Methods:
\vspace{-1em}
\begin{itemize}
	\small
	\item \textbf{RS}: random search
	\item \textbf{GP}: GP with the Tanimoto kernel
	\item \textbf{LA}: the Laplace-approximated MLP neural net
\end{itemize}

Foundation models/features:
\vspace{-1em}
\begin{itemize}
	\small
	\item \textbf{Fingerprints}: Molecular fingerprints baseline
	\item \textbf{Molformer}: Simple transformer over SMILES baseline
	\item \textbf{GPT2-M}: GPT2 Medium (345M params)
	\item \textbf{GPT2-L}: GPT2 Large (774M params)
	\item \textbf{Llama2-7B}: 7B params
	\item \textbf{T5-B}: T5-Base (220M params)
	\item \textbf{T5-B-Chem}: T5-B finetuned with chemistry data (220M params) \citep{christofidellis2023unifying}
\end{itemize}

Prompt types:
\vspace{-1em}
\begin{itemize}
	\small
	\item \textbf{just-smiles}: \emph{``\texttt{\{smiles\_str\}}''}
	      % \item \textbf{completion}: \emph{``The estimated redox potential of the molecule \texttt{\{smiles\_str\}} is: ''}
	      % \item \textbf{single-number}: \emph{``Answer with just numbers without any further explanation! What is the estimated redox potential of the molecule with the SMILES string \texttt{\{smiles\_str\}}?''}
\end{itemize}

Acquisition function: Thompson sampling---for a faithful assesment of the posterior.

\begin{figure}[h!]
	\centering

	\includegraphics[width=0.45\linewidth]{figs/redox-mer/fixed_feat_just-smiles-average}
	\includegraphics[width=0.45\linewidth]{figs/solvation/fixed_feat_just-smiles-average}

	\caption{
		Fixed-feature performance, i.e.\ the LLM is frozen and train only the last regression layer.
		The acquisition function is Thompson sampling.
	}
\end{figure}

\begin{summarybox}
	Even when the LLM is fixed \& the prompt is naive, its features are very informative.
	However, this only holds for the chemistry-specific LLM.
\end{summarybox}



\clearpage

\section*{Finding 2: Effects of prompting}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.5\linewidth]{figs/diagram_fixed_feat}

	\caption{\textbf{Source of uncertainty:} The  regressor, via the Laplace approximation. Already more principled than the uncertainty of ICL.}
\end{figure}

Prompt types:
\begin{itemize}
	\item \textbf{just-smiles}: \emph{``\texttt{\{smiles\_str\}}''}
	\item \textbf{completion}: \emph{``The estimated redox potential of the molecule \texttt{\{smiles\_str\}} is: ''}
	\item \textbf{single-number}: \emph{``Answer with just numbers without any further explanation! What is the estimated redox potential of the molecule with the SMILES string \texttt{\{smiles\_str\}}?''}
\end{itemize}

\begin{figure}[h!]
	\centering

	\includegraphics[width=0.45\linewidth]{figs/redox-mer/fixed_feat_just-smiles-average}
	\includegraphics[width=0.45\linewidth]{figs/redox-mer/fixed_feat_single-number-average}

	\includegraphics[width=0.45\linewidth]{figs/redox-mer/fixed_feat_completion-average}

	\vspace{-2em}
\end{figure}

\begin{figure}[h!]
	\centering

	\includegraphics[width=0.45\linewidth]{figs/solvation/fixed_feat_just-smiles-average}
	\includegraphics[width=0.45\linewidth]{figs/solvation/fixed_feat_single-number-average}

	\includegraphics[width=0.45\linewidth]{figs/solvation/fixed_feat_completion-average}

	\vspace{-2em}
\end{figure}

\begin{summarybox}
	General LLMs---LLAMA2, GPT2, T5---are not good.
	Domain-specific LLM is required for good results.
\end{summarybox}



\clearpage

\section*{Finding 3: Effects of finetuning}

Finetuning: LoRA is applied to the attention layers (query, value) of the foundation model.

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.5\linewidth]{figs/diagram_lora}

	\caption{
		\textbf{Source of uncertainty:} Both the adapted LLM \& the regression head. (Via the Laplace approximation.)
	}
\end{figure}


\begin{figure}[h!]
	\centering

	\includegraphics[width=0.45\linewidth]{figs/redox-mer/mixed_feat_just-smiles-average}
	\includegraphics[width=0.45\linewidth]{figs/solvation/mixed_feat_just-smiles-average}

	\caption{
		Finetuning performance. LoRA is used to adapt the LLM.
		The acquisition function is Thompson sampling.
	}
\end{figure}

\begin{summarybox}
	Additionally finetuning the LLM and taking into account the uncertainty of the finetuned LoRA weights \(\implies\) better results.
\end{summarybox}


\clearpage

\section*{Previous work}

\begin{itemize}
	\item Previous work, e.g.\ \citet{ramos2023bayesopticl,anonymous2023llambo} are using in-context learning (ICL).
	      \begin{itemize}
		      \item Prompting ChatGPT, e.g., \\
		            \emph{``I'm interested in estimating the redox potential of molecules, represented by their SMILES string. Here are some known data: \\
			            - SMILES: \texttt{\{smiles1\}}; redox potential: \texttt{\{redox1\}}, \\
			            - SMILES: \texttt{\{smiles2\}}; redox potential: \texttt{\{redox2\}}, \\
			            - SMILES: \texttt{\{smiles3\}}; redox potential: \texttt{\{redox3\}}. \\  Now, what is the estimated redox potential of \texttt{\{new\_smiles\}}?''}
	      \end{itemize}
	      %
	\item Their interpretation of \emph{Bayesian} optimization is quite ``liberal''
	      \begin{itemize}
		      \item \citet{ramos2023bayesopticl}: Using tokens' softmax probabilities as the uncertainty.
		      \item \citet{anonymous2023llambo}: The source of uncertainty is in the prompt templates. I.e., have \(k\) different prompts of the same data, then compute the variance of ChatGPT's answers.
	      \end{itemize}
	      %
	\item[] \(\implies\) They are just heuristic, and not principled BayesOpt methods.
	\item \textbf{Our goal:} Provide a way to do a principled BayesOpt with LLMs \& study our hypothesis.
\end{itemize}


\clearpage


\section*{Proposed story line}

\begin{enumerate}[(a)]
	\item \textbf{Motivation}
	      \begin{enumerate}[(i)]
		      \item LLMs seem useful for many task; their large sizes carry a lot of information. Might be useful as a prior for BayesOpt in molecular space.
		            %
		      \item From chemistry standpoint: \dots
		            %
		      \item Previous works are largely heuristic
	      \end{enumerate}
	      %
	\item \textbf{Contribution}
	      \begin{enumerate}[(i)]
		      \item Principled formulation of LLMs as surrogate functions in molecular BayesOpt.
		      \item A study of how the promises \& pitfalls of LLMs as surrogates.
		      \item Open source, easy to use implementation that accept any LLM
	      \end{enumerate}
	      %
	\item \textbf{Tentative messages/conclusions}
	      \begin{enumerate}[(i)]
		      \item Non-finetuned general LLMs are \emph{not} good as surrogates \(\implies\) raising questions of how reasonable are ICL-based methods
		            \begin{itemize}
			            \item (On top of them being unprincipled in terms of the uncertainty quantification.)
		            \end{itemize}
		            %
		      \item Domain-specific LLM is a good starting point. Finetuning generally improves performance.
		            \begin{itemize}
			            \item LLMs work actually because they have exposure to domain-related infos, i.e., standard transfer learning setup, not so much because of their ``intelligence''.
			            \item The above fit Occam's razor better; we verified empirically.
		            \end{itemize}
		            %
		      \item This is a good news: We don't need very large (expensive!) LLMs to get the best BayesOpt performance! T5-B-Chem is the smallest model here, only 220M params---everyone can do BayesOpt with LLMs!
		            %
		      \item Being Bayesian, in the LLM era, is not hard! No need for fancy yet kinda flawed uncertainty quantification heuristics.
	      \end{enumerate}
\end{enumerate}

\vfill\null

\subsection*{TO-DO:}
\begin{itemize}
	\item More baselines, esp.\ in-context learning \& GNN embedding.
	\item Evaluate on all datasets provided by Felix.
	\item Multi-objective optimization results.
\end{itemize}


\clearpage


\begin{figure*}
	\centering
	{\large \textbf{Redox-mer, t-SNE}}\par\vspace{1em}

	\begin{minipage}{0.24\textwidth}
		\includegraphics[width=\textwidth]{figs/redox-mer/dim_reduction/tsne_fingerprints}
	\end{minipage}
	%
	\begin{minipage}{0.725\textwidth}
		\includegraphics[width=\textwidth]{figs/redox-mer/dim_reduction/tsne_llm_feats}
	\end{minipage}

	\caption{
		t-SNE visualization of different embeddings (e.g., last hidden states of a LLM) for the \texttt{redox-mer} dataset.
		Red indicates the optimum.
		Rows indicate prompt types, columns indicate foundation models.
		The foundation model \textbf{t5-base-chem} is a chemistry-specific LLM by \citet{christofidellis2023unifying}.
		For prompt types,
		\textbf{just-smiles}: \emph{``\texttt{\{smiles\_str\}}''};
		\textbf{completion}: \emph{``The estimated redox potential of the molecule \texttt{\{smiles\_str\}} is: ''};
		\textbf{single-number}: \emph{``Answer with just numbers without any further explanation! What is the estimated redox potential of the molecule with the SMILES string \texttt{\{smiles\_str\}}?''}.
	}
\end{figure*}


\begin{figure*}
	\centering
	{\large \textbf{Redox-mer, UMAP}}\par\vspace{1em}

	\begin{minipage}{0.24\textwidth}
		\includegraphics[width=\textwidth]{figs/redox-mer/dim_reduction/umap_fingerprints}
	\end{minipage}
	%
	\begin{minipage}{0.725\textwidth}
		\includegraphics[width=\textwidth]{figs/redox-mer/dim_reduction/umap_llm_feats}
	\end{minipage}

	\caption{
		UMAP visualization of different embeddings (e.g., last hidden states of a LLM) for the \texttt{redox-mer} dataset.
		Red indicates the optimum.
		Rows indicate prompt types, columns indicate foundation models.
		The foundation model \textbf{t5-base-chem} is a chemistry-specific LLM by \citet{christofidellis2023unifying}.
		For prompt types,
		\textbf{just-smiles}: \emph{``\texttt{\{smiles\_str\}}''};
		\textbf{completion}: \emph{``The estimated redox potential of the molecule \texttt{\{smiles\_str\}} is: ''};
		\textbf{single-number}: \emph{``Answer with just numbers without any further explanation! What is the estimated redox potential of the molecule with the SMILES string \texttt{\{smiles\_str\}}?''}.
	}
\end{figure*}



\begin{figure*}
	\centering
	{\large \textbf{Redox-mer, t-SNE, Average}}\par\vspace{1em}

	\begin{minipage}{0.24\textwidth}
		\includegraphics[width=\textwidth]{figs/redox-mer/dim_reduction/tsne_fingerprints}
	\end{minipage}
	%
	\begin{minipage}{0.725\textwidth}
		\includegraphics[width=\textwidth]{figs/redox-mer/dim_reduction/tsne_llm_feats_average}
	\end{minipage}

	\caption{
		t-SNE visualization of different embeddings (e.g., last hidden states of a LLM) for the \texttt{redox-mer} dataset.
		Red indicates the optimum.
		Rows indicate prompt types, columns indicate foundation models.
		The foundation model \textbf{t5-base-chem} is a chemistry-specific LLM by \citet{christofidellis2023unifying}.
		For prompt types,
		\textbf{just-smiles}: \emph{``\texttt{\{smiles\_str\}}''};
		\textbf{completion}: \emph{``The estimated redox potential of the molecule \texttt{\{smiles\_str\}} is: ''};
		\textbf{single-number}: \emph{``Answer with just numbers without any further explanation! What is the estimated redox potential of the molecule with the SMILES string \texttt{\{smiles\_str\}}?''}.
	}
\end{figure*}


\begin{figure*}
	\centering
	{\large \textbf{Redox-mer, UMAP, Average}}\par\vspace{1em}

	\begin{minipage}{0.24\textwidth}
		\includegraphics[width=\textwidth]{figs/redox-mer/dim_reduction/umap_fingerprints}
	\end{minipage}
	%
	\begin{minipage}{0.725\textwidth}
		\includegraphics[width=\textwidth]{figs/redox-mer/dim_reduction/umap_llm_feats_average}
	\end{minipage}

	\caption{
		UMAP visualization of different embeddings (e.g., last hidden states of a LLM) for the \texttt{redox-mer} dataset.
		Red indicates the optimum.
		Rows indicate prompt types, columns indicate foundation models.
		The foundation model \textbf{t5-base-chem} is a chemistry-specific LLM by \citet{christofidellis2023unifying}.
		For prompt types,
		\textbf{just-smiles}: \emph{``\texttt{\{smiles\_str\}}''};
		\textbf{completion}: \emph{``The estimated redox potential of the molecule \texttt{\{smiles\_str\}} is: ''};
		\textbf{single-number}: \emph{``Answer with just numbers without any further explanation! What is the estimated redox potential of the molecule with the SMILES string \texttt{\{smiles\_str\}}?''}.
	}
\end{figure*}

